ShaSTA: Modeling Shape and Spatio-Temporal Affinities for 3D Multi-Object Tracking

Multi-object tracking is a cornerstone capability of any robotic system. The quality of tracking is largely dependent on the quality of the detector used. In many applications, such as autonomous vehicles, it is preferable to over-detect objects to avoid catastrophic outcomes due to missed detections. As a result, current state-of-the-art 3D detectors produce high rates of false-positives to ensure a low number of false-negatives. This can negatively affect tracking by making data association and track lifecycle management more challenging. Additionally, occasional false-negative detections due to difficult scenarios like occlusions can harm tracking performance. To address these issues in a unified framework, we propose to learn shape and spatio-temporal affinities between tracks and detections in consecutive frames. Our affinity provides a probabilistic matching that leads to robust data association, track lifecycle management, false-positive elimination, false-negative propagation, and sequential track confidence refinement. Though past 3D MOT approaches address a subset of components in this problem domain, we offer the first self-contained framework that addresses all these aspects of the 3D MOT problem. We quantitatively evaluate our method on the nuScenes tracking benchmark where we achieve 1st place amongst LiDAR-only trackers using CenterPoint detections. Our method estimates accurate and precise tracks, while decreasing the overall number of false-positive and false-negative tracks and increasing the number of true-positive tracks. We analyze our performance with 5 metrics, giving a comprehensive overview of our approach to indicate how our tracking framework may impact the ultimate goal of an autonomous mobile agent. We also present ablative experiments and qualitative results that demonstrate our framework's capabilities in complex scenarios.

==> figures/modules.tex <==
\newdimen\figrasterwd
\figrasterwd\textwidth


\begin{figure*}[thpb!]
  \centering
  \parbox{\figrasterwd}{
    \parbox{.45\figrasterwd}{
      \subcaptionbox{\label{fig:mod_1}}{\includegraphics[width=\hsize]{canon_box_module.png}}
      \subcaptionbox{\label{fig:mod_2}}{\includegraphics[width=\hsize]{canon_shape_module_v2.png}}
    }
    \hspace{2em}
    \parbox{.5\figrasterwd}{%
      \subcaptionbox{\label{fig:mod_3}}{
      \centering
      \includegraphics[width=\hsize]{figures/src/residual_module_v2.png}}
      \subcaptionbox{\label{fig:mod_4}}{\includegraphics[width=\hsize]{aff_module.png}}
    }
  }
  \caption{Algorithm Modules. \textcolor{red}{TODO: WRITE CAPTION}}
\label{fig:module}
\end{figure*}

==> figures/teaser.tex <==
% \begin{figure*}[th!]
%     \centering
%     \begin{subfigure}[t]{0.45\linewidth}
%       \centering
%       \includegraphics[width=0.45\linewidth]{figures/src/teaser_v3.png}
%       \caption{In Frame 0, we initialize the newborn track for bounding box 1 (yellow). In the next frame, we successfully track the yellow car over time with bounding box 1, while we initialize another newborn track for the red car with bounding box 2. Finally, in the third frame, we continue to correctly track the red car, and we kill track 1.}
%       \label{fig:teaser1}
%     \end{subfigure}
%     \hspace{2em}
%     % \vspace{1cm}
%     \begin{subfigure}[t]{0.5\linewidth}
%       \centering
%       \includegraphics[width=0.5\linewidth]{figures/src/teaser_v3_p2.png}
%       \caption{In the second frame, we did not successfully track the yellow car, and thus, have a false-negative for bounding box 1. In the third frame, the affinity matrix shows that bounding box 3 is a false-positive, as there is no object where the box is predicted.}
%       \label{fig:teaser2}
%     \end{subfigure}
%     \caption{We illustrate with two examples how the affinity matrix is defined per frame.}
%     \label{fig:teaser}
% \end{figure*}


\newdimen\figrasterwd
\figrasterwd\textwidth


\begin{figure*}[thpb!]
  \centering
  \parbox{\figrasterwd}{
    \parbox{.48\figrasterwd}{
      \subcaptionbox{\label{fig:teaser1}}{\includegraphics[width=\hsize]{figures/src/teaser_v3.png}}
    }
    \hspace{2em}
    \parbox{.48\figrasterwd}{%
      \subcaptionbox{\label{fig:teaser2}}{
      \centering
      \includegraphics[width=\hsize]{figures/src/teaser_v3_p2.png}}
    }
  }
  \caption{Illustration of Affinity Matrix. \textcolor{red}{TODO: WRITE CAPTION}}
\label{fig:module}
\end{figure*}


==> sections/related-work-legacy.tex <==
\section{Related Work}

\subsection{3D Object Detection on LiDAR Point Clouds}
\textbf{Please note: I copy-pasted parts from colton's paper, since it covers what I want to discuss here. I will work on paraphrasing this later.}

3D detection is one of the most important modules for most 3D tracking frameworks. While 3D detectors from camera data have seen recent improvement \cite{kehl2017ssd, liu2020smoke, park2021pseudo}, LiDAR-based 3D detection offers much better performance, especially in driving scenes \cite{engelcke2017vote3deep, ge2020afdet, lang2019pointpillars, shi2020pv, yin2021center, zhou2018voxelnet}. The majority of works on LiDAR-based detection have centered around improving feature extraction from unorganized point clouds. On the one hand, VoxelNet \cite{zhou2018voxelnet} groups points by 3D voxels and extracts voxel-level features using PointNet \cite{qi2017pointnet}. PointPillar \cite{lang2019pointpillars} organizes point clouds in vertical columns (pillars) to achieve higher efficiency. On the other hand, CenterPoint \cite{yin2021center} improves the 3D detector by looking at the output representation, proposing a point-based object representation at the decoding stage. While our proposed approach is not constrained to a specific input detector, we use CenterPoint detections in our experiments due to its popularity and to facilitate comparison with other state-of-the-art tracking algorithms.

In addition to improving the 3D detector architecture, aggregating temporal information has also been shown to improve 3D detection results as it compensates for the sparsity of LiDAR sensor inputs. nuScenes \cite{caesar2020nuscenes} devises a simple way to accumulate multiple LiDAR sweeps with motion compensation, providing a richer point cloud with an added temporal dimension. Using accumulated point clouds is shown to improve the overall performance for multiple detector architectures \cite{lang2019pointpillars, zhu2019class} and enables more exploration of object visibility reasoning \cite{hu2020you}.


\subsection{2D Multi-Object Tracking}
In the 2D domain, image-based multi-object tracking is the dominating paradigm, since images provide rich information that includes color, texture, and other appearance cues that aid in track formation and association \cite{dan2019, leal2016learning, chang2019online, zeng2021motr, sun2020transtrack, meinhardt2022trackformer}. Siamese networks \cite{leal2016learning, chang2019online} have been proven to be robust to medium- and long-term occlusions. Transformer-based techniques that employ a tracking-by-attention approach \cite{zeng2021motr, sun2020transtrack, meinhardt2022trackformer}, as opposed to following the tracking-by-detection paradigm, combine the detection and tracking problem into one solution, whereby data association is completed implicitly with static object queries that function as detections for newborn objects, while track queries are updated autoregressively. In these techniques, even though initializing newborn tracks integrates information learned by the model, killing tracks is only based on heuristics. Finally, \cite{dan2019} learns affinity matrices between consecutive frames by finding correlations between 2D image features encoded from each frame with VGG \cite{simonyan2014very}.

\subsection{3D Multi-Object Tracking}
\textbf{Please note: I copy-pasted parts from colton's paper and voxelnet, since they cover what I want to discuss here. I will work on paraphrasing this later.}

Thanks to the advances in 3D object detection discussed above, most state-of-the-art 3D MOT algorithms follow the tracking-by-detection paradigm. The performance of 3D MOT algorithms is mainly affected by three factors other than detection results: the motion prediction model, the association metric, and the life-cycle management of the tracklets.
CenterPoint \cite{yin2021center} proposes a simple, yet effective, approach that gives reliable detection results and estimates velocities to propagate detections between sequential frames. The distance between object centers is used as the association metric.
The most popular category of 3D MOT algorithms leverages Kalman Filters to estimate the location of tracked objects and their dynamics, providing predictions for future association. AB3DMOT \cite{weng2019baseline} provides the prior baseline in this direction and leverages 3D Intersection-over-Union (IoU) as the association metric. Following this line, \cite{kuang2020probabilistic} proposes to replace 3D IoU with the Mahalanobis distance to better capture the uncertainty of the tracklets.

There are also several multi-modal fusion methods that
combine images and LiDAR to improve accuracy \cite{chiu2021probabilistic, chen2017multi, enzweiler2011multilevel, gonzalez2016board}. These methods provide improved performance compared to LiDAR-only 3D detection, particularly for small objects (pedestrians) or when the objects are far, since cameras provide an order of magnitude more measurements than LiDAR. However the need for an additional camera that is time synchronized and calibrated with the LiDAR restricts their use and makes the solution more sensitive to sensor failure modes. In this work we focus on LiDAR-only tracking and use LiDAR-only input detections.

